Efficient Explanations for Knowledge Compilation Languages

Knowledge compilation (KC) languages find a growing number of practical uses, including in Constraint Programming (CP) and in Machine Learning (ML). In most applications, one natural question is how to explain the decisions made by models represented by a KC language. This paper shows that for many of the best known KC languages, well-known classes of explanations can be computed in polynomial time. These classes include deterministic decomposable negation normal form (d-DNNF), and so any KC language that is strictly less succinct than d-DNNF. Furthermore, the paper also investigates the conditions under which polynomial time computation of explanations can be extended to KC languages more succinct than d-DNNF.

==> acks.tex <==

\paragraph{Acknowledgments.} This work was supported by the AI
Interdisciplinary Institute ANITI, funded by the French program
``Investing for the Future -- PIA3'' under Grant agreement
no.\ ANR-19-PI3A-0004, and by the H2020-ICT38 project COALA
``Cognitive Assisted agile manufacturing for a Labor force supported
by trustworthy Artificial intelligence''.


==> texfigs/table-ddnnf.tex <==
\setlength{\tabcolsep}{5pt}
\rowcolors{2}{gray!10}{}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}

\begin{table*}[t]%[h]
\centering
\resizebox{\textwidth}{!}{
  \begin{tabular}{l>{\lpr}S[table-format=4.0,table-space-text-pre=\lpr]S[table-format=3.0,table-space-text-post=\rpr]<{\rpr}S[table-format=2.0]c  c cccc  cccc  cccc}
\toprule[1.2pt]
\rowcolor{white}

\multirow{2}{*}{\bf Dataset} & \multicolumn{2}{c}{\multirow{2}{*}{\bf (\#F~~~~\#S)}}  & \multicolumn{2}{c}{\bf sd-DNNF} & \multicolumn{1}{c}{\bf XPs}  & \multicolumn{4}{c}{\bf AXp} & \multicolumn{4}{c}{\bf CXp}  &  \multicolumn{4}{c}{\bf Runtime~(s)}\\

  \cmidrule[0.8pt](lr{.75em}){4-5}
  \cmidrule[0.8pt](lr{.75em}){6-6}
  \cmidrule[0.8pt](lr{.75em}){7-10}
  \cmidrule[0.8pt](lr{.75em}){11-14}
  \cmidrule[0.8pt](lr{.75em}){15-18} 
  %
\rowcolor{white}
& \multicolumn{2}{c}{}   & {\bf \#N} & {\bf \%A}  &  {\bf avg} & {\bf M} &  {\bf m} & {\bf avg} & {\bf \%L} &  {\bf M} &  {\bf m} & {\bf avg} & {\bf \%L} & {\bf Tot}  & {\bf M}  & {\bf m} &  {\bf avg}  \\
\toprule[1.2pt]
corral & 6 & 160 & 35 & 100 & 4 & 4 & 1 & 2 & 34 & 4 & 2 & 2 & 22 & 0.231 & 0.004 & 0.001 & 0.001 \\
db-bodies & 4702 & 64 & 22 & 100 & 4 & 3 & 1 & 2 & 1 & 4 & 1 & 3 & 1 & 0.144 & 0.004 & 0.001 & 0.002 \\
db-bodies-stemmed & 3721 & 64 & 14 & 84.6 & 4 & 2 & 1 & 1 & 1 & 4 & 1 & 2 & 1 & 0.125 & 0.003 & 0.001 & 0.002 \\
db-subjects & 242 & 64 & 45 & 84.6 & 6 & 4 & 1 & 2 & 2 & 6 & 3 & 4 & 1 & 0.153 & 0.005 & 0.001 & 0.002 \\
db-subjects-stemmed & 229  & 64 & 54 & 92.3 & 7 & 4 & 1 & 2 & 2 & 7 & 2 & 5 & 1 & 0.190 & 0.006 & 0.001 & 0.003 \\
mofn\_3\_7\_10 & 10 & 1324 & 107 & 97.7 & 11 & 28 & 1 & 4 & 32 & 28 & 2 & 6 & 24 & 14.476 & 0.072 & 0.002 & 0.011 \\
mux6 & 6 & 128 & 62 & 100 & 5 & 4 & 1 & 2 & 51 & 4 & 3 & 3 & 24 & 0.411 & 0.009 & 0.001 & 0.003 \\
parity5+5 & 10 & 1124 & 484 & 85.7 & 9 & 12 & 1 & 2 & 66 & 19 & 5 & 7 & 14 & 43.144 & 0.193 & 0.015 & 0.038 \\
spect & 22 & 267 & 108 & 85.1 & 14 & 36 & 1 & 8 & 22 & 13 & 2 & 6 & 10 & 8.062 & 0.105 & 0.005 & 0.030 \\
threeOf9 & 9 & 512 & 76 & 96.1 & 7 & 15 & 1 & 3 & 38 & 14 & 3 & 4 & 19 & 3.079 & 0.023 & 0.002 & 0.006 \\
xd6 & 9 & 973 & 80 & 97.9 & 8 & 25 & 1 & 4 & 36 & 22 & 3 & 4 & 20 & 8.657 & 0.035 & 0.002 & 0.009 \\
\bottomrule[1.2pt]
\end{tabular}
}
\caption{\footnotesize{Listing all  AXps  CXps for sd-DNNFs. 
%
Columns {\bf \#F} and {\bf \#S} report, resp., the number of features 
and the number of tested samples, in the dataset. 
Column {\bf XPs}  reports  the average number of total explanations 
(AXp's and CXp's). 
Sub-Columns {\bf \#N} and {\bf \%A} show, resp., the total number of 
nodes and test accuracy of the sd-DNNF.
Sub-columns {\bf M},  {\bf m} and {\bf avg} of column {\bf AXp} 
(resp.,  {\bf CXp}) show, resp., the maximum, minimum and average 
number of explanations. The average length (as a percentage of \#F) of an explanation  (AXp/CXp) is given 
as {\bf \%L}.
Sub-columns  {\bf Tot}, {\bf M},  {\bf m} and {\bf avg}  of column {\bf Runtime} 
report, resp., the total, maximal, minimal and average run time (in seconds) 
to list all the explanations for all tested instances.
}}
\label{tab:ddnnf}
\end{table*}



==> texfigs/table-sdd.tex <==

\begin{table*}[t]%[h]
\centering
\resizebox{\textwidth}{!}{
  \begin{tabular}{l>{\lpr}S[table-format=4.0,table-space-text-pre=\lpr]S[table-format=3.0,table-space-text-post=\rpr]<{\rpr}S[table-format=2.0]c  c cccc  cccc  cccc}
\toprule[1.2pt]
\rowcolor{white}
\multirow{2}{*}{\bf Dataset} & \multicolumn{2}{c}{\multirow{2}{*}{\bf (\#F~~~~\#S)}}  & \multicolumn{2}{c}{\bf SDD} & \multicolumn{1}{c}{\bf XPs}  & \multicolumn{4}{c}{\bf AXp} & \multicolumn{4}{c}{\bf CXp}  &  \multicolumn{4}{c}{\bf Runtime~(s)}\\
  \cmidrule[0.8pt](lr{.75em}){4-5}
  \cmidrule[0.8pt](lr{.75em}){6-6}
  \cmidrule[0.8pt](lr{.75em}){7-10}
  \cmidrule[0.8pt](lr{.75em}){11-14}
  \cmidrule[0.8pt](lr{.75em}){15-18} 
  %
\rowcolor{white}
& \multicolumn{2}{c}{}   & {\bf \#N} & {\bf \%A}  &  {\bf avg} & {\bf M} &  {\bf m} & {\bf avg} & {\bf \%L} &  {\bf M} &  {\bf m} & {\bf avg} & {\bf \%L} & {\bf Tot}  & {\bf M}  & {\bf m} &  {\bf avg}  \\
\toprule[1.2pt]
corral & 6 & 160 & 12 & 100 & 4 & 4 & 1 & 2 & 34 & 4 & 2 & 2 & 22 & 0.057 & 0.001 & 0.000 & 0.000 \\
dw-bodies & 4702 & 64 & 21 & 100 & 4 & 3 & 1 & 2 & 1 & 4 & 1 & 3 & 1 & 0.026 & 0.001 & 0.000 & 0.000 \\
dw-bodies-stemmed & 3721 & 64 & 15 & 84.6 & 4 & 2 & 1 & 1 & 1 & 4 & 1 & 2 & 1 & 0.025 & 0.001 & 0.000 & 0.000 \\
dw-subjects & 242 & 64 & 28 & 84.6 & 6 & 4 & 1 & 2 & 2 & 6 & 3 & 4 & 1 & 0.090 & 0.004 & 0.000 & 0.001 \\
dw-subjects-stemmed & 229  & 64 & 31 & 92.3 & 7 & 4 & 1 & 2 & 2 & 7 & 2 & 5 & 1 & 0.099 & 0.004 & 0.001 & 0.002 \\
mofn\_3\_7\_10 & 10 & 1324 & 34 & 97.7 & 11 & 28 & 1 & 4 & 32 & 28 & 2 & 6 & 24 & 1.692 & 0.008 & 0.000 & 0.001 \\
mux6 & 6 & 128 & 22 & 100 & 5 & 4 & 1 & 2 & 51 & 4 & 3 & 3 & 24 & 0.081 & 0.002 & 0.000 & 0.001 \\
parity5+5 & 10 & 1124 & 96 & 85.7 & 9 & 12 & 1 & 2 & 66 & 19 & 5 & 7 & 14 & 2.269 & 0.009 & 0.000 & 0.002 \\
spect & 22 & 267 & 55 & 85.1 & 14 & 36 & 1 & 8 & 22 & 13 & 2 & 6 & 10 & 1.238 & 0.016 & 0.001 & 0.005 \\
threeOf9 & 9 & 512 & 37 & 96.1 & 7 & 15 & 1 & 3 & 38 & 14 & 3 & 4 & 19 & 0.596 & 0.005 & 0.000 & 0.001 \\
xd6 & 9 & 973 & 36 & 97.9 & 8 & 25 & 1 & 4 & 36 & 22 & 3 & 4 & 20 & 1.147 & 0.007 & 0.000 & 0.001 \\
\bottomrule[1.2pt]
\end{tabular}
}
\caption{\footnotesize{Listing all AXps and CXps for SDDs. 
%
%Sub-Columns {\bf \#N} and {\bf \%A} report, respectively,
%total number of nodes and test accuracy of a SDD.
%The remaining columns have the same meaning as described in the caption of \autoref{tab:ddnnf}.
(Note that, \autoref{tab:sdd}'s columns have the same meaning as described in the caption of \autoref{tab:ddnnf}.)
}} 
\label{tab:sdd}
\end{table*}

